A differentiable Gaussian Prototype Layer for explainable Segmentation

We introduce a Gaussian Prototype Layer for gradient-based prototype learning and demonstrate two novel network architectures for explainable segmentation one of which relies on region proposals. Both models are evaluated on agricultural datasets. While Gaussian Mixture Models (GMMs) have been used to model latent distributions of neural networks before, they are typically fitted using the EM algorithm. Instead, the proposed prototype layer relies on gradient-based optimization and hence allows for end-to-end training. This facilitates development and allows to use the full potential of a trainable deep feature extractor. We show that it can be used as a novel building block for explainable neural networks. We employ our Gaussian Prototype Layer in (1) a model where prototypes are detected in the latent grid and (2) a model inspired by Fast-RCNN with SLIC superpixels as region proposals. The earlier achieves a similar performance as compared to the state-of-the art while the latter has the benefit of a more precise prototype localization that comes at the cost of slightly lower accuracies. By introducing a gradient-based GMM layer we combine the benefits of end-to-end training with the simplicity and theoretical foundation of GMMs which will allow to adapt existing semi-supervised learning strategies for prototypical part models in future.

==> deleted.tex <==
. Recent research addresses various aspects of prototype based Deep Learning: Case based reasoning and deep prototype vectors \cite{li2018deep}, ProtoPNet \cite{chen2019looks}, Multiple sets of prototypes to learn a taxonomy \cite{hase2019interpretable}, Fitting prototypes with an iterative scheme \cite{chong2021towards}.\\
Here we use differentiable GMMs for explainable image segmentation. Deep gaussian mixture models for robustness \cite{yang2018robust}. Deep Gaussian Autoencoders for Anomaly detection \cite{zong2018deep}
Gradient based training of high dimensional Gaussian Mixture Models \cite{gepperth2021gradient} Outlier detection.
PyKeOps \cite{charlier2021kernel}
// Deep Gaussian Prototypes
Multiple Object Tracking and Segmentation \cite{ke2021prototypical}
//Texture segmentation
// Discrete key value bottleneck


While ProtoPNet uses a hard assignment of image patches to prototypes a more recent model employs expectancy maximization (EM) to fit the kernels of a Gaussian Mixture Model (GMM) iteratively\cite{ke2021prototypical}.



We evaluate our explainable segmentation models on two datasets from the agricultural domain: The MinneApple dataset that contains semantic segmentation of apples in an orchard and WGISD with segmented grapes. To ensure a good comparability with other state-of-the-art approaches for semantic segmentation of fruits we compare to two common methods for image segmentation that have also already been employed for fruit segmentation before. An approach that classifies super-pixels based on their color as well as variations of UNet with deep feature extractors\cite{hani2020minneapple}. Table 1 summarizes all results. \\




Hence we demonstrate prototypes with attributed bounding boxes and gradient based training of a deep prototype network with a GMM layer. Prototype learning is not only suited for classification but also for explainable segmentation which is especially important in the agricultural domain\cite{trauble2022discrete}.

%\
Moving ahead of classification we show that a gradient based Gaussian Prototype Layer can serve as a building block in networks for semantic segmentation and in combination with region proposals. In future this may help to enable new modes of human AI interaction.


Most commonly prototype networks are used to classify images and identify charactersitic visual features of the classes. Differences exist regarding the way prototypes are fitted, using iterative or gradient-based schemes with prototype pruning or without, the question if negative reasoning is allowed or prohibited the backbone (CNNs, GNNs  or transformers) and whether relationships between prototypes such as taxonomies or configurations in pixel space are modeled.


Differences exist regarding the way prototypes are fitted, using iterative or gradient-based schemes with prototype
pruning or without, the question if negative reasoning is allowed or prohibited, the backbone (CNNs
GNNs [13] or transformers) and whether relationships between prototypes such as taxonomies or configurations in pixel space are modeled.


The cost term weights the distance between $p_j$ and $p_s$ logarithmically decreasing and is maximal if antitype and a prototype coincide. It thus encourages the prototypes to diverge from latent encodings of non-object patches. The antitype vectors are initialized with the prototypes that the user identifies as non-object. The prototoypes diverge from the antitypes that are inserted by the user due to the repelling term in the loss. \Figref{user_interaction} illustrates this process.

\newcolumntype{C}{>{\centering\arraybackslash}X} % centered version of "X" type
\setlength{\extrarowheight}{1pt}

==> my_table.tex <==
\begin{table*}
 \caption{Evaluation Matrices (Case Study 1)}
\label{my-label}
\begin{tabularx}{\textwidth}{@{}l*{10}{C}c@{}}
\toprule

Encoder     & Covariance Type & Kernels  & TP & FP & TN & FN & AUC \\ 
\midrule
HSV     & spherical & 128          & 17   & 19  & 3    & 1   &     10    \\ 
        & spherical & 256          & 17   & 19  & 3    & 1   &     10    \\ 
        & full        & 128        & 3    & 4   & 0    & 0   & 3    &    \\ 
        & full        & 256        & 3    & 4   & 0    & 0   & 3    &    \\ 
\addlinespace
AlexNet     & spherical & 128          & 17   & 19  & 3    & 1   &     10    \\ 
        & spherical & 256          & 17   & 19  & 3    & 1   &     10    \\ 
        & full        & 128        & 3    & 4   & 0    & 0   & 3    &    \\ 
        & full        & 256        & 3    & 4   & 0    & 0   & 3    &    \\ 
\addlinespace
ResNet32     & spherical & 128          & 17   & 19  & 3    & 1   &     10    \\ 
        & spherical & 256          & 17   & 19  & 3    & 1   &     10    \\ 
        & full        & 128        & 3    & 4   & 0    & 0   & 3    &    \\ 
        & full        & 256        & 3    & 4   & 0    & 0   & 3    &    \\ 
\bottomrule
\end{tabularx}
\end{table*}

